Deciding Linear Height and Linear Size-to-Height Increase for Macro Tree Transducers

We present a novel normal form for (total deterministic) macro tree transducers (mtts), called depth proper normal form. If an mtt is in this normal form, then it is guaranteed that each parameter of each state of the mtt appears at arbitrary depth in the output trees of that state. Intuitively, if some parameter only appears at certain bounded depths in the output trees of a state, then this parameter can be removed by in-lining the corresponding output paths at each call site of that state. We use regular look-ahead in order to determine which of the paths should be in-lined. As a consequence of changing the lookahead, a parameter that was previously appearing at unbounded depths, may be appearing at bounded depths for some new look-ahead; for this reason, our construction has be iterated in order to obtain an mtt in depth-normal form. Using the normal form, we can decide whether the translation of an mtt has linear height increase or has linear size-to-height increase.

==> ICALP_preliminaries.tex <==
%!TEX root = ICALP_main.tex
\section{Preliminaries}
\label{sect:prelim}

The set $\{0,1,\dots \}$ of natural numbers is denoted by $\mathbb{N}$.
For $k\in\mathbb{N}$ we denote by $[k]$ the set
$\{1,\dots,k\}$; thus $[0]=\emptyset$.
A ranked alphabet (set) consists of an alphabet (set) $\Sigma$ together
with a mapping $\text{rank}_{\Sigma}: \Sigma\to\mathbb{N}$
that assigns each symbol $\sigma\in\Sigma$ a natural number called its ``rank''.
We write $\sigma^{(k)}\in\Sigma$ to denote that $\sigma\in\Sigma$ and
$\text{rank}_{\Sigma}(\sigma)=k$.
By $\Sigma^{(k)}$ we denote the symbols of $\Sigma$ that have rank $k$.
%
The set $T_\Sigma$ of (finite, ranked, ordered) trees over $\Sigma$ is the smallest
set $S$ such that if $\sigma\in\Sigma^{(k)}$, $k\geq 0$, and
$s_1,\dots,s_k\in S$, then also $\sigma(s_1,\dots,s_k)\in S$.
We write $\sigma$ instead of $\sigma()$.
For a tree $s=\sigma(s_1,\dots,s_k)$ with $\sigma\in\Sigma^{(k)}$, $k\geq 0$,
and $s_1,\dots,s_k\in T_\Sigma$, we define 
the set $V(s)\subseteq\mathbb{N}^*$ of nodes of $s$ as
$\{\varepsilon\}\cup \{ iu\mid i\in[k], u\in V(s_i)\}$;
thus, nodes are strings over positive integers.
Thus, $\varepsilon$ denotes the root node of $s$, and
for a node $u$, $ui$ denotes the $i$-th child of $u$.
For $u\in V(s)$ we denote by $s[u]$ the label of $u$ in $s$ and
by $s/u$ the subtree rooted at $u$.
Formally, let $s=\sigma(s_1,\dots,s_k)$ and define 
$s[\epsilon]=\sigma$,
$s[iu]=s_i[u]$, 
$s/\varepsilon=s$, and
$s/iu=s_i/u$ for $\sigma\in\Sigma^{(k)}$, $k\geq 0$,
$s_1,\dots,s_k\in T_\Sigma$, $i\geq 1$ and $u\in V(s_i)$ such that $iu\in V(s)$.

We fix two special sets of symbols: the set $X=\{x_1,x_2,\dots \}$ of
variables and the set $Y=\{y_1,y_2,\dots\}$ of parameters.
For $k\geq 1$ let $X_k=\{x_1,\dots,x_k\}$ and $Y_k=\{y_1,\dots,y_k\}$.
Let $A$ be a set that is disjoint from $\Sigma$. Then the set $T_\Sigma(A)$ of
trees over $\Sigma$ indexed by $A$ is defined as $T_{\Sigma'}$ where
$\Sigma'=\Sigma\cup A$ and $\text{rank}_{\Sigma'}(a)=0$ for $a\in A$ and 
$\text{rank}_{\Sigma'}(\sigma)=\text{rank}_{\Sigma}$ for $\sigma\in\Sigma$.

For a ranked alphabet $\Sigma$ and a set $A$ the ranked set
$\<\Sigma,A>$  consists of all symbols $\<\sigma,a>$ with $\sigma\in\Sigma$ and
$a\in A$; the rank of $\<\sigma,a>$ is defined as $\text{rank}_\Sigma(\sigma)$.

\medskip

%\subsection{Tree Substitutio}n
\textbf{Tree Substitution.}\quad
Let $\Sigma$ be a ranked alphabet and let $s,t\in T_\Sigma$.
For $u\in V(s)$ we define the tree $s[u\leftarrow t]$ that is obtained
from $s$ by replacing the subtree rooted at node $u$ by the tree $t$.
Let $\sigma_1,\dots,\sigma_n\in\Sigma^{(0)}$, $n\geq 1$ be pairwise distinct symbols
and let $t_1,\dots,t_n\in T_\Sigma$. Then $t[\sigma_i\leftarrow t_i\mid i\in[n]]$
is the tree obtained from $t$ by replacing each occurrence of $\sigma_i$ by
the tree $t_i$. We have defined trees as particular strings, and this is just
ordinary string substitution (because we only replace symbols of rank zero).
We refer to this as ``first-order tree substitution''.

In ``second-order tree substitution'' it is possible to replace internal nodes $u$ (of a tree $s$)
by new trees. These new trees use parameters to indicate where
the ``dangling'' subtrees $s/ui$ of the node $u$ are to be placed.
Let $\sigma_1\in\Sigma^{(k_1)},\dots, \sigma_n\in\Sigma^{(k_n)}$ be pairwise distinct symbols 
with $n\geq 1$ and
$k_1,\dots,k_n\in\mathbb{N}$ and let $t_i\in T_\Sigma(Y_{k_i})$ for $i\in[n]$.
Let $s\in T_\Sigma$.
Then $s[\![\sigma_i\leftarrow t_i\mid i\in[n]]\!]$ denotes the tree
that is inductively defined as (abbreviating $[\![\sigma_i\leftarrow t_i\mid i\in[n]]\!]$ by
$[\![\dots ]\!]$) follows:
for $s=\sigma(s_1,\dots,s_k)$,
if $\sigma\not\in\{\sigma_1,\dots,\sigma_n\}$ then $s[\![\dots]\!]=\sigma(s_1[\![\dots]\!],
\dots,s_k[\![\dots]\!])$ and if $\sigma=\sigma_j$ for some $j\in[n]$ then
$s[\![\dots]\!]=t_j[y_i\leftarrow s_i[\![\dots]\!]\mid i\in[k]]$.

\medskip 

%\subsection{Macro Tree Transducers}
%\label{sect:mtt}
\textbf{Macro Tree Transducers.}\quad
A (deterministic bottom-up) \emph{tree automaton} $A$ is given by a tuple
$(P,\Sigma,h)$ where $P$ is a finite set of states, $\Sigma$ is a ranked alphabet,
and $h$ is a collection of mappings $h_\sigma:P^k\to P$ with $\sigma\in\Sigma^{(k)}$
and $k\geq 0$ such that the collection is surjective (i.e., for every $p\in P$ there
exists a $\sigma$ such that $p$ is in the range of $h_\sigma$).
The extension of $h$ to a mapping $\hat{h}:T_\Sigma\to P$
is defined recursively as $\hat{h}(\sigma(s_1,\dots,s_k))=
h_\sigma(\hat{h}(s_1),\dots,\hat{h}(s_k))$ for every $\sigma\in\Sigma^{(k)}$,
$k\geq 0$, and $s_1,\dots,s_k$. For every $p\in P$ we define the subset $L_p$ of trees
in $T_\Sigma$ as $\{ s\in T_\Sigma\mid \hat{h}(s)=p\}$.
Note that $L_p\not=\emptyset$ due to the surjectivity requirement above.

A (total, deterministic) \emph{macro tree transducer with (regular) look-ahead} (``mttr'') 
$M$ is given by a tuple
$(Q,P,\Sigma,\Delta,q_0,R,h)$, where
\begin{itemize}
\item $Q$ is a ranked alphabet of \emph{states},
\item $\Sigma$ and $\Delta$ are ranked alphabet of \emph{input} and \emph{output symbols},
\item $(P,\Sigma,h)$ is a tree automaton (called the \emph{look-ahead automaton} of $M$),
\item $q_0\in Q^{(0)}$ is the \emph{initial state},
\item and $R$ is the \emph{set of rules}, where for each $q\in Q^{(m)}$, $m\geq 0$,
$\sigma\in\Sigma^{(k)}, k\geq 0$, and $p_1,\dots, p_k\in P$ there is exactly one rule of the form 
\[
\<q,\sigma(x_1:p_1,\dots,x_k:p_k)>(y_1,\dots,y_m) \to t
\]
with $t\in T_{\Delta\cup \< Q,X_k>}(Y_m)$.
The right-hand side $t$ of such a rule is denoted by
$\text{rhs}_M(q,\sigma,\<p_1, \dots,p_k>)$
\end{itemize}

We use a notation that is slightly different from the one used in the Introduction:
instead of, e.g., $q_2(x_2, q_{\text{id}}(x_1))$ we write
$\< q_2,x_2>(\< q_{\text{id}},x_1>)$.
Thus, we use angular brackets $\< \dots >$ to indicate a state call on an input subtree,
and use round brackets (after the angular brackets), to indicate the parameter arguments
of the particular state call.

The semantics of an mttr $M$ (as above) is defined as follows.
We define the derivation relation $\Rightarrow_M$ as follows.
For two trees $\xi_1,\xi_2\in T_{\Delta\cup\< Q,T_\Sigma>}(Y)$,
$\xi_1\Rightarrow_M\xi_2$ if there exists a node $u$ in $\xi_1$
with $\xi_1/u=\<q,s>(t_1,\dots,t_m)$, $q\in Q^{(m)}$, $m\geq 0$,
$s=\sigma(s_1,\dots,s_k)$, $\sigma\in\Sigma^{(k)}$, $k\geq 0$,
$s_1,\dots,s_k\in T_\Sigma$,
$t_1,\dots,t_m\in T_{\Delta\cup\<Q,T_\Sigma>}(Y)$, and 
$\xi_2=\xi_1[u\leftarrow\xi]$ where $\xi$ equals
\[
\zeta
[\![\<q',x_i>\leftarrow \<q',s_i>\mid q'\in Q,i\in[k]]\!]
[y_j\leftarrow t_j\mid j\in[m]]
\]
and $\zeta=\text{rhs}_M(q,\sigma,\<\hat{h}(s_1),\dots,\hat{h}(s_k)>)$.
Since $M$ is total (i.e.,
for every state $q$, input symbol $\sigma\in\Sigma^{(k)}$, $k\geq 0$, and 
look-ahead states $p_1,\dots,p_k$, $M$ contains a corresponding rule)
%and $\Rightarrow_M$ is confluent and terminating,
there is for every $\xi_1$ a unique
tree $\xi'\in T_\Delta(Y)$ such that $\xi_1\Rightarrow_M^* \xi'$.
For every $q\in Q^{(m)}$, $m\geq 0$ and $s\in T_\Sigma$ we define the
\emph{$q$-translation of $s$}, denoted by $M_q(s)$, as the unique tree $t$ in $T_\Delta(Y_m)$ such that
$\<q,s>(y_1,\dots, y_m)\Rightarrow_M^* t$.
We denote the \emph{translation realized by $M$} also by $M$, i.e., 
$M=M_{q_0}$ and for every $s\in T_\Sigma$,
$M(s)=M_{q_0}(s)$ is the unique tree $t\in T_\Delta$
such that $\< q_0,s>\Rightarrow_M^* t$.

Let $M$ be an mttr as before.
We define \emph{the extension $\widehat{M}$ of $M$} which can also process
look-ahead states at leaves of input trees.
Let $\widehat{M}=(Q,P,\hat{\Sigma},\hat{\Delta},q_0,R\cup \hat{R},h\cup h')$ where
$\hat{\Sigma}=\Sigma\cup \{p^{(0)}\mid p\in P\}$ and
$\hat{\Delta}=\Delta\cup \{\< q,p>^{(m)} \mid q \in Q^{(m)}, p \in P, m\geq 0\}$.
For every $q\in Q^{(m)}$, $m\geq 0$, and $p\in P$ we let $h(p)=p$ and we
let the rule
$\<q,p>(y_1, \dots, y_m)\to \<q,p>(y_1, \dots, y_m)$ be in $\hat{R}$;
note that the $\<q,p>$ on the right-hand side of this rule is an output symbol.
%
For the original transducer $M$ we say that the pair $(q,p)$ is
\emph{reachable (in $M$)} if there is an input tree $s\in T_{\hat{\Sigma}}$ such
that $\<q,p>$ occurs in $\widehat{M}(s)$.
Clearly it is decidable for a given pair $(q,p)$, whether or not
it is reachable; this is because (1)~inverse translations of mttrs
effectively preserve regularity~\cite{DBLP:journals/jcss/EngelfrietV85,DBLP:journals/ipl/PerstS04},
(2)~the set of all trees in $T_{\hat{\Delta}}$
that contain at least one occurrence of $\< q,p>$ is regular, and
(3)~emptiness of regular tree languages is decidable~\cite{TATA07}. 

We say that $M$ is \emph{nondeleting}, if for every state $q\in Q^{(m)}$,
$m\geq 1$, $\sigma\in\Sigma^{(k)}, k\geq 0$, $p_1,\dots, p_k\in P$,
and $j\in[m]$, there is at least one occurrence of $y_j$ in
$\text{rhs}_M(q,\sigma,\< p_1,\dots,p_k>)$.
The next proposition is proved in~\cite[Lemma~6.7]{DBLP:journals/iandc/EngelfrietM99}
(for mttrs that do not copy parameters, but the proof works analogously for
arbitrary mtts).

\begin{proposition}
\label{prop:nondeleting}
For every mttr, an equivalent nondeleting mttr $M$ can be constructed such that,
for every state $q$ of $M$ of rank $m\geq 1$ and
for every $j\in[m]$ it holds that $M_q(s)$ contains at least one
occurrence of $y_j$, for every $s\in T_\Sigma$.
\end{proposition}

It is well known that the finiteness of ranges of compositions of 
mttrs is decidable~\cite{DBLP:journals/iandc/DrewesE98}.
A (partial nondeterministic) top-down tree transducer with look-ahead
(``topr'' for short)
is an mttr
as before, where $Q=Q^{(0)}$ and $R$ may contain none or several
rules for each given $q$ and $\sigma$.


\begin{proposition}(\cite[Theorem~4.5]{DBLP:journals/iandc/DrewesE98})
\label{prop:finite}
For a given composition of mttrs and (partial nondeterministic) toprs it is 
decidable whether or not the range of the composition is finite. 
In the case of finiteness, the range can be constructed.
\end{proposition}

%Note that a ``partial'' mttr is one where for some $q,\sigma,p_1,\dots,p_k$
%it may be that $\text{rhs}_M(q,\sigma,\< p_1,\dots,p_k>)$ is \emph{not}
%defined.


==> conclusions.tex <==
\section{Conclusions}

We have proven that for a given macro tree transducer (with look-ahead) it
is decidable whether or not it has linear height increase (LHI) and,
whether or not it has linear size-to-height increase (LSHI).
Both decision procedures rely on a novel normal form that is called
``depth-proper'' normal form. Roughly speaking the normal form requires
that each parameter of every state of the transducer appears at
arbitrary large depth in output trees generated by that state (and for a given
look-ahead state). Our construction
of the normal form removes parameters that only appear at bounded depth. 
Once in depth-normal form, we can reduce the check for LHI and LSHI
to the finiteness of ranges of mtts.

Both LHI and LSHI are natural properties and have several useful applications.
For instance, if an mtt does not have LHI, then we know that it cannot be realized
by a top-down or a bottom-up tree transducer. And, if an mtt does not have LSHI, then
we know that it cannot be realized by any attributed tree transducers.
%
%The most prevailing open problem is to solve the conjecture (see Introduction) that
%the translation of an mtt can be realized by an attributed tree transducer if and only
%if the translation is of LSOI (linear size-to-number-of-distinct-output-subtrees).
%In this paper we merely show that \emph{deciding} if an mtt is of LSOI is as
%hard as deciding equivalence of attributed transducers (a long standing difficult open problem).
%We believe that the depth-proper normal form will be helpful in solving the conjecture.
%Intuitively, loops need to be considered only if they produce an arbitrary number of copies of
%states with parameters. In these loops we can exclude certain state nestings, due to
%the normal form.
%
An interesting open problem is the question whether or not the mtt hierarchy
(generated by sequential compositions of mtts) collapses for LSHI or for LHI.
By this we mean (in the case of LSHI), whether or not there exists some number $n$ such that
$
\cup \{ \text{MTT}^k \mid k\geq 1 \} \cap \text{LSHI} \subseteq \text{MTT}^n.
$
Note that for linear size increase, the hierarchy collapses~\cite{DBLP:journals/acta/EngelfrietIM21}
to level one, i.e., $n=1$.
It can be shown by an easy counting argument (similar as when proving that sequential composition
of mttrs gives rise to a hierarchy that is strict at each level) that no such $n$ exists:
consider compositions of the translation $\tau$ that takes a binary
tree $s$ as input and outputs a full binary tree of height $|s|$.
Then $\tau_k\in
\text{MTT}\cap\text{LSHI})^{k+1} - \text{MTT}\cap\text{LSHI})^k$.
Thus, the MTT hierarchy restricted to linear size-to-height increase remains to
be strict at each level.

The corresponding question for LHI is open, i.e., we do not know whether or not
the MTT hieararchy restricted to linear height increase is strict.
We do have a candidate translation that would show (for level two) both, that a two-fold composition of
mtts of LHI can do strictly more than a single mtt, and, that two-fold compositions
that are of LHI are strictly more than a single mtt:
input trees are monadic trees of the form $a^n(e)$ and output trees are full binary
trees of height $n$, at the leaves of which are monadic trees that represent
the Dewey paths of those ``leaves'' of the binary tree.
E.g.
$a(a(e))$ is translated to
$
f(f(1(1(e)), 1(2(e))), f(2(1(e)), 2(2(e)))).
$
Note that if we output \emph{reverse} such Dewey paths, then the translation
indeed can be realized by a single mtt (see, e.g., Fig.~6.2 in~\cite{DBLP:series/eatcs/FulopV98}).
Thus, the second transducer of the composition reverses the reverse Dewey paths.

\newpage

==> constr_plus_examples.tex <==
\subsection{Construction of the Normal Form and Examples}
\label{sect:examples}

%\subsection{Formal Construction of the Depth Proper Normal Form}
%\label{sect:dp}

Let $M$ be an mttr as before. 
We assume that $M$ is nondeleting (which is justified by 
Proposition~\ref{prop:nondeleting}).
The idea of the construction is as follows.
First, we determine all reachable pairs $(q,p)$ 
such that $Y(q,p)\not=\emptyset$.
Let $(q,p)$ be such a pair and let $Z=Y(q,p)$.
An occurrence of $\<q,x_i>$ in a right-hand side
$\text{rhs}_M(q',\sigma,\< p_1,\dots,p_k>)$ such that $p_i=p$ is
called a \emph{$(q,p)$-call}. Our aim is to replace each $(q,p)$-call
by an appropriate tree from $\lcop{M_q(L_p)}_Z$. Just which tree is
the appropriate one will be determined by regular look-ahead. 
Moreover, such trees should be modified not to contain leaf nodes 
labeled by subsets of $Y$: such nodes will be replaced by 
calls of new ``helper states''. 

We now present the formal construction of the transducer $\pi(M)$.
Note that in general, $\pi(M)$ is \emph{not} depth proper yet, but
the construction needs to be iterated several times (cf. the examples in
Section~\ref{sect:examples}).

\begin{definition}
\label{df:pi}
Let $M=(Q,P,\Sigma,\Delta,q_0,R,h)$ be a nondeleting mttr
that is not depth proper.
We construct the new mttr
$\pi(M)=(Q\cup H,P',\Sigma,\Delta,q_0,R',h')$.
% The sets $H$ and $P'$ are defined as follows.
For every 
$q\in Q^{(m)}$, $m\geq 1$, and $p\in P$ such that $Y(q,p)\not=\emptyset$,
$H$ contains the following set of helper states:
\[
\{ [q,p,t,u]^{(|U|)}\mid 
t\in \lcop{M_q(L_p)}_{Y(q,p)}, 
u\in V(t),
t/u=U\subseteq Y_m \}
\]
and $P'$ contains $(p,\varphi)$ for any
function $\varphi$ that assigns to each $q\in F_p$ 
a tree in $\lcop{M_q(L_p)}_{Y(q,p)}$.
%
Observe that $H$ and $P'$ are well defined, because
$\lcop{M_q(L_p)}_{Y(q,p)}$ is finite by Lemma~\ref{lm:lcop_finite}. 
%
Note that $|U|\leq |Y_m \setminus Y(q,p)|$; since $Y(q,p)$ is non-empty this implies that
the rank of each helper state is at most $(r-1)$, where $r$ is the maximal
rank of the states in $Q$. 

For every $q\in Q^{(m)}$, $m\geq 0$, 
$\sigma\in\Sigma^{(k)}$, $k\geq 0$, and 
$(p_1,\varphi_1),\dots,(p_k,\varphi_k)\in P'$ we let the rule
\[
\<q,\sigma(x_1:(p_1,\varphi_1),\dots,x_k:(p_i,\varphi_i)>(y_1,\dots,y_m)
\to\text{rhs}_M(q,\sigma,\<p_1,\dots,p_k>)[\![ . ]\!]
\]
be in $R'$, where the second-order tree substitution
$[\![ . ]\!]$ is defined as follows.
\begin{multline*}
[\![ . ]\!] = 
[\![\< q',x_i>\leftarrow \varphi_i(q')\big[
u\leftarrow [q',p_i,\varphi_i(q'),u](y_{j_1},\dots,y_{j_n})\mid \\
\varphi_i(q')/u=\{y_{j_1},\dots,y_{j_n}\},
j_1<\cdots <j_n\big] \mid q'\in F_{p_i}, i\in[k]
 ]\!].
\end{multline*}
We define $h_\sigma'((p_1,\varphi_1),\dots,(p_k,\varphi_k))=(p,\varphi)$
where $p=h_\sigma(p_1,\dots,p_k)$ and, using special second-order substitution 
from Definition~\ref{def:meta-skeleta}, for every $q\in F_p$,  
\[
\varphi(q)=
\lcop{
\text{rhs}_M(q,\sigma,\<p_1,\dots,p_k>)
[\![\< q',x_i>\leftarrow \varphi_i(q')\mid q'\in F_{p_i}, i\in[k]]\!]\su
}_{Y(q,p)}.
\]
%
For every helper state $[q,p,t,u]\in H^{(n)}$, $n\geq 0$,
$\sigma\in\Sigma^{(k)}$, $k\geq 0$, and 
$(p_1,\varphi_1),\dots,$ $(p_k,\varphi_k)\in P'$ 
such that $h_\sigma(p_1,\dots,p_k)=p$
we let the rule
\[
\<[q,p,t,u](\sigma(x_1:(p_1,\varphi_1),\dots,x_k:(p_k,\varphi_k))>(y_1,\dots,y_n)
\to \xi/u[y_{j_\nu}\leftarrow y_\nu\mid\nu\in[n]]
\]
be in $R'$ where
$t/u=\{y_{j_1},\dots,y_{j_n}\}$,
$j_1<\cdots <j_n$,
$\xi=\text{rhs}_M(q,\sigma,\<p_1,\dots,p_k>)[\![ . ]\!]$, and
$[\![ . ]\!]$ is the substitution from above.
\end{definition}

\input{example}



==> construction.tex <==
%!TEX root = main.tex
\section{Depth Proper Normal Form}

The depth proper normal form requires that each parameter of
each state $q$ occurs at unbounded depth in the output trees of that state 
(for each given look-ahead state $p$ such that $(q,p)$ is reachable).
Formally, let $q$ be a state of rank $m\geq 1$, $j\in[m]$, and
$p\in P$. 
If $(q,p)$ is reachable, then 
for every natural number $n$ there must exist an input tree $s_n \in L_p$ such that
$y_j$ occurs at depth $>n$ in the tree $M_q(s_n)$.
Conversely, we say that parameter $y_j$ is \emph{depth-bounded} for $q$ and $p$ 
if there exists an $n$ for which no such input tree $s_n \in L_p$ exists;
more generally, we say that $Z\subseteq Y_m$ is
\emph{depth-bounded} for $q$ and $p$, if each $y\in Z$ is depth-bounded for $q$ and $p$.

If $Z$ is depth-bounded for $q$ and $p$, then there are only finitely many output paths
in the trees in $M_q(L_p)$ under which the parameters from $Z$ occur.
The \emph{$Z$-skeleton} of an arbitrary tree $t$ is obtained from $t$
by replacing each top-most node $u$ such that $t/u$ does not contain any
occurrence of a parameter from $Z$ by some symbol. 
Clearly, $Z$ is depth-bounded for $q$ and $p$ if and only if the $Z$-skeleta of
all trees in $M_q(L_p)$ form a finite set.

Let $\Delta$ be an arbitrary ranked alphabet, $m\geq 1$, 
$t\in T_\Delta(Y_m)$, and $Z\subseteq Y_m$.
Let us write \(\paras{t}\subseteq{Y_m}\) for the set of parameters 
occurring in $t$.
Let us now be more specific as to which symbols replace the top-most nodes $u$
of $t$ such that $\paras{t/u}\cap Z=\emptyset$. Since in our construction later
we will want to obtain a transducer that is nondeleting, it will be helpful
to know which parameters appear in a given deleted tree. Therefore we replace
such nodes $u$ by the set $\paras{t/u}$. 
We denote by $\lcop{t}_Z$ the $Z$-skeleton of $t$ and define it inductively as follows
(where $\delta\in\Delta$):
\begin{align*}
\lcop{t}_Z &= 
\begin{cases}
t &
\text{if \(t\in Z\)}
\\
\delta(\lcop{t_1}_Z,\dots,\lcop{t_n}_Z) &
\text{if \(\paras{t}\cap Z\ne\emptyset\) and \(t = \delta(t_1,\dots,t_n)\)}
\\
\paras{t} & \text{if \(\paras{t}\cap Z = \emptyset\)}.
\end{cases}
\end{align*}

The definition of $\lcop{t}_Z$ is extended to sets $L$ of trees
as $\lcop{L}_Z=\{\lcop{t}_Z\mid t\in L\}$.
We call \emph{$Y$-nodes} the nodes $u$ in $V(\lcop{t}_Z)$ such 
that $\lcop{t}_Z/u=Z'\subseteq Y_m$. We denote by 
$\mathcal{U}(\lcop{t}_Z)$ the set of $Y$-nodes on $\lcop{t}_Z$. 
The notion of parameters in a tree naturally extends to $Z$-skeleta with, 
for a $Y$-node labeled $Z'$: $\paras{Z'} = Z'$. 

\begin{lemma}\label{lm:nd}
Let $\Delta$ be a ranked alphabet, $m\geq 1$, $Z\subseteq Y_m$, and
$t\in T_\Delta(Y_m)$.
(1)~$t=\lcop{t}_Z[u\leftarrow t/u\mid u\in\mathcal{U}(\lcop{t}_Z)]$.
(2)~$\paras{\lcop{t}_Z} = \paras{t}$. 
%(3)~If $y\in Y_m$ occurs in $t$, then 
%there exists a leaf $u\in V(\lcop{t}_Z)$
%such that either $\lcop{t}_Z/u=y$ or 
%$\lcop{t}_Z/u=Z'\subseteq Y_m$ and $y\in Z'$.
\end{lemma}
\begin{proof}
The proof is by induction on the structure of $\lcop{t}_Z$.
Let us denote the substitution $[u\leftarrow t/u\mid u\in\mathcal{U}(\lcop{t}_Z)]$
by $[t]$.
%
There are three cases.

Case 1: $t = y\in Z$. Then $\mathcal{U}(\lcop{t}_Z)=\emptyset$.
Hence $\lcop{t}_Z[t]=\lcop{y}_Z$. The latter equals $y=t$ by 
the definition of $\lcop{.}_Z$. Thus~(1)~holds. Also 
$\paras{\lcop{t}_Z}=\{y\}=\paras{t}$ and so~(2)~holds. 
%the definition of $\lcop{.}_Z$. Thus~(1)~holds and~(2)~holds for $u=\epsilon$.

Case 2: $\paras{t} \cap Z = \emptyset$. Then $\lcop{t}_Z = \paras{t} = Z' \subseteq Y_m$ 
by the definition of $\lcop{.}_Z$, and $\mathcal{U}(\lcop{t}_Z)=\{ \epsilon \}$. Hence
$\lcop{t}_Z[t] = \lcop{t}_Z[\epsilon\leftarrow t/\epsilon = t] = t$ which proves~(1). 
Again~(2)~holds 
because $\paras{\lcop{t}_Z}=\paras{\paras{t}}=\paras{t}$. 
%for $u=\varepsilon$ for each $y \in \paras{t}$ i.e.\ $y$ occurring in $t$.

Case 3: \(\paras{t}\cap Z\ne\emptyset\). Then $t=\delta(t_1,\dots,t_n)$, 
$\delta\in\Delta^{(n)}$, $n\geq 0$,
and $t_1,\dots, t_n\in T_\Delta(Y_m)$.
To show~(1) we obtain from the definition of $\lcop{t}_Z$ that
\[
\lcop{t}_Z[t]=\delta(\lcop{t_1}_Z,\dots,\lcop{t_n}_Z)[t]
= \delta(\lcop{t_1}_Z[t_1],\dots,\lcop{t_n}_Z[t_n]),
\]
where for $i\in[n]$, $[t_i]$ denotes the substitution
$[u\leftarrow t_i/u\mid u\in\mathcal{U}(\lcop{t_i}_Z)]$.
By induction the latter equals $\delta(t_1,\dots,t_n)=t$.
Finally~(2)~is implied by the induction hypothesis:
$\paras{\lcop{t}_Z}=\bigcup_{j\in[n]} \paras{\lcop{t_j}_Z}
=\bigcup_{j\in[n]} \paras{t_j}= \paras{t}$
%To show~(2), assume $y\in Y_m$ occurs in $t$.
%Thus, $n\geq 1$ and there exists an $i\in[n]$
%such that $y$ occurs in $t_i$.
%By induction of Statement~(2), there exists a leaf $u$ of $t_i$ such that 
%Statement~(2) holds (for $u$ and $t_i$); therefore Statement~(2) holds
%for $iu$ and $t$.
\qed


%%Sebastian's version:
%The proof is by induction on the structure of $t$.
%Let us denote the substitution $[u\leftarrow t/u\mid u\in\mathcal{U}(\lcop{t}_Z)]$
%by $[t]$.
%%
%We first consider $t=y\in Y$. There are two cases.
%
%Case 1: $y\in Z$. Then $\mathcal{U}(\lcop{t}_Z)=\emptyset$.
%Hence $\lcop{t}_Z[t]=\lcop{y}_Z$. The latter equals $y=t$ by 
%the definition of $\lcop{.}_Z$. Thus~(1)~holds and~(2)~holds for $u=\epsilon$.
%
%Case 2: $y\not\in Z$. Then $\mathcal{U}(\lcop{t}_Z)=\{ \epsilon \}$ and hence
%$\lcop{t}_Z[t] = \lcop{t}_Z[\epsilon\leftarrow t/\epsilon = t] = t$ which proves~(1).
%Moreover, $\lcop{t}_Z=\{y_j\}$ by the definition of $\lcop{.}_Z$,
%i.e., again~(2)~holds for $u=\varepsilon$.
%
%Now consider $t=\delta(t_1,\dots,t_n)$, $\delta\in\Delta^{(n)}$, $n\geq 0$,
%and $t_1,\dots, t_n\in T_\Delta(Y_m)$.
%To show~(1) we obtain from the definition $\lcop{t}_Z$ that
%\[
%\lcop{t}_Z[t]=\delta(\lcop{t_1}_Z,\dots,\lcop{t_n}_Z)[t]
%= \delta(\lcop{t_1}_Z[t_1],\dots,\lcop{t_n}_Z[t_n]),
%\]
%where for $i\in[n]$, $[t_i]$ denotes the substitution
%$[u\leftarrow t_i/u\mid u\in\mathcal{U}(\lcop{t_i}_Z)]$.
%By induction the latter equals $\delta(t_1,\dots,t_n)=t$.
%To show~(2) we assume that $y_j$ occurs in $t$ for some $j\in[m]$.
%Thus, $n\geq 1$ and there exists an $i\in[n]$
%such that $y_j$ occurs in $t_i$.
%By the induction for Statement~(2), there exists a leaf $u$ of $t_i$ such that 
%the Statement~(2) holds (for $u$ and $t_i$), and therefore Statement~(2) holds
%for $iu$ and $t$.
\end{proof}

Finally, we define depth properness for mtts with look-ahead. 

\begin{definition} \label{df_depth_proper}
The mttr $M=(Q,P,\Sigma,\Delta,q_0,R,h)$ is in \emph{depth proper normal form}
(or, synonymously, $M$ is \emph{depth proper})
if for every $q\in Q^{(m)}$, $m\geq 1$, and $p\in P$ it holds that
if $(q,p)$ is reachable, then  
$\lcop{M_q(L_p)}_{\{y_j\}}$ is infinite for all $j\in[m]$.
\end{definition}

From now on we will want to make use of the following definitions:
\[
\begin{array}{lcl}
F_p &=& \{ q\in Q^{(m)}\mid \exists j\in[m], \lcop{M_q(L_p)}_{\{y_j\}}
\text{ is finite}\}\\
Y(q,p) &=& \{ y_j\mid j\in[\text{rank}_Q(q)]\text{ such that }
\lcop{M_q(L_p)}_{\{y_j\}}\text{ is finite}\}
\end{array}
\]

It should be clear that $\lcop{M_q(L_p)}_{Y(q,p)}$ is finite for every $q$ and $p$,
as shown in the next lemma.

\begin{lemma}\label{lm:lcop_finite}
Let $M$ be an mtt, $q$ a state of $M$, and $p$ a look-ahead state of $M$
such that $Y(q,p)\not=\emptyset$.
Then $\lcop{M_q(L_p)}_{Y(q,p)}$ is finite.
\end{lemma}
\begin{proof}
Assume that $Y_{q,p}=\{y_{j_1},\dots,y_{j_n}\}$ where $n\geq 1$.
It follows from the definition of $Y(q,p)$ that for each $i\in[n]$ there exists
a number $d_i$ such that $y_{j_i}$ occurs at depth $\leq d_i$ in 
any tree in $M_q(L_p)$. Let $d$ be the maximum of all numbers in
$\{ d_1,\dots,d_n\}$. Then every parameter in $Y(q,p)$ occurs at depth $\leq d$ in
any tree in $M_q(L_p)$. It follows from the definition of $U=\lcop{M_q(L_p)}_{Y(q,p)}$
that every node of a tree in $U$ has depth $\leq d$. Thus, $U$ is finite.
\qed
\end{proof}

Before we proceed with the construction of the depth proper normal form,
we want to be able to decide whether or not a given mttr is depth proper.

%\newpage

\subsection{Deciding whether or not a given Mttr is Depth Proper}

In this section we prove that for a given mttr it is decidable whether or
not it is depth proper.
Moreover, we present a technical lemma giving properties of parameters and 
skeleta of state-calls appearing in right-hand-sides of rules. 
%states that if a certain
%parameter is depth proper and appears nested in the right-hand side of a rule,
%then a parameter of the nested state is depth proper as well. 

\begin{lemma}\label{lm:dec}
Let $M=(Q,P,\Sigma,\Delta,q_0,R,h)$ be an mttr and let
$q\in Q^{(m)}$, $m\geq 1$, $j\in[m]$, and $p\in P$.
It is decidable whether or not 
$\lcop{M_q(L_p)}_{\{y_j\}}$ is finite.
In case of finiteness, 
$\lcop{M_q(L_p)}_{\{y_j\}}$ can be constructed.
\end{lemma}
\begin{proof}
Let $Z=\{y_j\}$.
We now consider symbols in $Y_m$ as rank zero symbols.
It is straightforward to construct a  top-down tree transducer with look-ahead $M_Z$ which outputs
$\lcop{t}_Z$ for input trees $t\in T_{\Delta\cup Y_m}$; note that
$T_{\Delta\cup Y_m}=T_\Delta(Y_m)$ because symbols in $Y_m$ are now considered
as symbols of rank zero.
The transducer $M_Z$ computes in its look-ahead $h'$ the set of parameters of
the input tree, i.e.\ $h'(t)=\paras{t}$ for every $t\in T_{\Delta\cup Y_m}$. 
The transducer $M_Z$ (which consists of a single state only) outputs $\paras{t}$
as soon as $\paras{t}\cap Z=\emptyset$.
%The details can be found in the Appendix.

Formally, $M_Z = (\{q_1^{(0)}\},P',\Delta\cup Y_m,\Delta',q_1,R',h')$ where
$P'={\cal P}(Y_m)$ and
$\Delta'=\Delta\cup \{ S^{(0)}\mid S\in P'\}\cup Y_m$.
For $y\in Y_m$ let $h'_y()=\{y\}$ and for
$a\in\Delta^{(0)}$ let $h'_a()=\emptyset$.
Further, for $\delta\in\Delta^{(k)}$, $k\geq 1$, and 
$S_1,\dots,S_k\in P'$ let 
$h'_\delta(S_1,\dots,S_k)=\bigcup_{i\in[k]}S_i$.
For $a\in\Delta^{(0)}$ let the rule
$\< q_1,a>\to\emptyset$ be in $R$.
Let $y\in Y_m$.
If $y\in Z$ then let the rule
$\< q_1,y>\to y$ be in $R$ and otherwise let the rule
$\< q_1,y>\to \{y\}$ be in $R$.
For $\delta\in\Delta^{(k)}$ with $k\geq 1$ 
and $S_1,\dots,S_k\in P'$
we define the rule
$\< q_1,\delta(x_1:S_1,\dots,x_k:S_k)>\to\zeta$ where $\zeta$ is defined as:
\[
\begin{array}{lcll}
  \zeta & = &
\left\{ 
  \begin{array}{ll}
  S & \text{if }S= (\bigcup_{i\in[k]} S_i)\cap Z=\emptyset\\
  \delta(\< q_1,x_1>,\dots,\<q_1,x_k>) & \text{otherwise.}
  \end{array}
\right. 
\end{array}
\]

\noindent
\textbf{Claim.}\quad
For every $t\in T_{\Delta\cup Y_m}$, $h'(t)=\paras{t}$ and
$M_Z(t)=\lcop{t}_Z$.

\medskip

It is straightforward to prove this claim by induction on the structure of $t$.
By the Claim,
$M_{\{y_j\}}(M_q(L_p)) = \lcop{M_q(L_p)}_{\{y_j\}}$.
The tree language $L_p$ can be represented by a partial nondeterministic
top-down tree transducer that realizes the identity on trees in $L_p$
(and is undefined otherwise; its rules are obtained by reading the
definitions of $h$ from right to left). 
In this way $M_{\{y_j\}}(M_q(L_p))$ is represented
so that its finiteness is decidable by Proposition~\ref{prop:finite}
(and in case of finiteness the set can be constructed).
\qed
\end{proof}

Since for a pair $(q,p)$ it is decidable whether or not it is reachable
(see Section~\ref{sect:mtt}), Lemma~\ref{lm:dec} implies that
it is decidable whether or not a given mttr is depth proper.
We conclude this section with a small lemma showing that
the skeleton of the output of an mttr \(M\) can be directly computed
from given a input tree 
by modifying the rules of \(M\).
%given a 
%right-hand-side of rule $t$, the skeleton of $t$ can be computed from the 
%skeleta of state calls appearing in $t$. 
For this lemma we first need to define how to compute second-order 
substitutions of skeleta,
which will be used for the modification of the right-hand sides of rules.
We do so on a \emph{nondeleting} mttr $M$, 
i.e.\ such that states always use all their parameters. 

\begin{definition}\label{def:meta-skeleta}
%Let $M$ be a nondeleting mttr as before. 
  %
Let $\Gamma$ be a ranked alphabet
 and
let $t_1,\dots,t_n\in T_\Gamma(Y)$. 
Let $s\in T_\Gamma(Y_n\cup\mathcal{P}(Y_n))$. 
%
%\begin{itemize}
%\item
%\item Let \(k_i = 0\) for all \(i\in[n]\).
The \emph{special first-order substitution} 
$[y_i \leftarrow t_i \mid i \in [n]]\su$ (for short $[.]\su$) applied to $s$ is
inductively defined as:
\begin{align*}
	s[.]\su &= 
	\begin{cases}
		t_i &
%		\text{if \(s=\gamma_i\) for \(i\in [n]\)}
		\text{if \(s=y_i\) for \(i\in [n]\)}
		\\
		\gamma(s_1[.]\su,\dots,s_k[.]\su) &
%		\text{if \(s = \gamma(s_1,\dots,s_k)\) and }\gamma\not\in\{\gamma_1,\dots,\gamma_n\}
		\text{if \(s = \gamma(s_1,\dots,s_k)\)}
		\\
		\bigcup_{i\in U} \paras{t_i} & \text{if \(s= \{y_i \mid i\in U\} \subseteq Y_n\)
                  for some \(U \subseteq [n]\).}
%		\bigcup_{y_i \in t'} \paras{t_i} & \text{if \(t' \subseteq Y_{m'}\) is a sequence node}.
	\end{cases}
\end{align*}

%For all pairwise distinct symbols $\sigma_1\in\Delta^{(k_1)},\dots, 
%\sigma_n\in\Delta^{(k_n)}$ with $n\geq 1$ and
%$k_1,\dots,k_n\in\mathbb{N}$ and let $t_i$ for $i\in[n]$.
%Let $s\in T_\Delta$.
%Then $s[\![\sigma_i\leftarrow t_i\mid i\in[n]]\!]$ denotes the tree
%that is inductively defined as (abbreviating $[\![\sigma_i\leftarrow t_i\mid i\in[n]]\!]$ by
%$[\![\dots ]\!]$) follows:
%for $s=\sigma(s_1,\dots,s_k)$,
%if $\sigma\not\in\{\sigma_1,\dots,\sigma_n\}$ then $s[\![\dots]\!]=\sigma(s_1[\![\dots]\!],
%\dots,s_k[\![\dots]\!])$ and if $\sigma=\sigma_j$ for some $j\in[n]$ then
%$s[\![\dots]\!]=t_j[y_i\leftarrow s_i[\![\dots]\!]\mid i\in[k]]$.
%\item
Let $\gamma_1^{(k_1)},\dots,\gamma_n^{(k_n)}\in\Gamma$, $n\geq 1$ be pairwise different symbols
%Let $k_i=rank_\Gamma(\gamma_i)$ for $i\in[n]$
and assume now that 
$t_i\in T_\Gamma(Y_{k_i}\cup\mathcal{P}(Y_{k_i}))$ for $i\in[n]$
and that $s\in T_\Gamma(Y_n)$. 
%
The \emph{special second-order substitution} 
$[\![\gamma_i \leftarrow t_i\mid i\in[n]]\!]\sp{}$
(for short $[\![.]\!]\su$) applied to $s$ is
%inductively defined as 
%if $s=\gamma(s_1, \dots, s_k)$
%with $\gamma\not\in\{\gamma_1,\dots,\gamma_n\}$
%then $s[\![.]\!]\su = 
%\gamma(s_1[\![.]\!]\su, \dots, s_k[\![.]\!]\su)$, 
%if $s=y_j$ for $j\in [n]$ then $s[\![.]\!]\su = s$, 
%and if $s=\gamma_i$ for $i\in[n]$ then
%$s[\![.]\!]\su =  t_i
%[y_j \leftarrow t_j[\![.]\!]\su \mid j \in [n]]\su$. 
inductively defined as:
\begin{align*}
s[\![.]\!]\su &=
\begin{cases}
t_i
[y_j \leftarrow s_j[\![.]\!]\su \mid j \in [k_i]]\su
&
\text{if $s=\gamma_i(s_1, \dots, s_{k_i})$ for $i\in[n]$}
\\
\gamma(s_1[\![.]\!]\su, \dots, s_k[\![.]\!]\su)
& \text{if $s=\gamma(s_1, \dots, s_k)$
with $\gamma\not\in\{\gamma_1,\dots,\gamma_n\}$}
\\
s
&
\text{if $s=y_j$ for $j\in [n]$.}
\end{cases}
\end{align*}
%if $s=\gamma(s_1, \dots, s_k)$
%with $\gamma\not\in\{\gamma_1,\dots,\gamma_n\}$
%then $s[\![.]\!]\su = 
%\gamma(s_1[\![.]\!]\su, \dots, s_k[\![.]\!]\su)$, 
%if $s=y_j$ for $j\in [n]$ then $s[\![.]\!]\su = s$, 
%and if $s=\gamma_i$ for $i\in[n]$ then
%$s[\![.]\!]\su =  t_i
%[y_j \leftarrow t_j[\![.]\!]\su \mid j \in [n]]\su$. 

For all sets $Z \subseteq Y_m$ such that no $Y$-node in 
$t[\![.]\!]\su$ intersects $Z$, we define the $Z$-skeleton 
$\lcop{t[\![.]\!]\su}_Z$ of $t[\![.]\!]\su$ inductively as 
before, with a special case for $Y$-nodes: for all $Y$-nodes $S$ we 
have $\lcop{S}_Z = S \subseteq Y_m \setminus Z$. 
%\end{itemize}
\end{definition}

%Old version of the end of the definition of compatibility of rhs
%To define this notion of compatibility, we consider the second-order 
%substitution of a state call (in the right-hand-side of a rule) with the 
%state's skeleton, which induces a 
%first-order substitution of the parameters in the skeleton. We take such 
%first-order substitutions to apply \emph{within} sequence nodes of the skeleton 
%so that, given a sequence node $S=\{y_1,y_3\}$: 
%$S[y_i \leftarrow t_i]_{i\in [3]} = \{t_1,t_3\}$. 
%We assume given an mttr $M$ as before, with the condition that 
%$M$ is \emph{nondeleting}, which 
%means that all parameters of a state are used to build the state's output.
%
%\begin{definition}\label{def:meta-skeleta}
%For all states $q \in Q^{(m)}, q'\in Q^{(m')}$, $\sigma\in\Sigma^{(k)}$, 
%and $p_1,\dots,p_k\in P$, and noting $p=h(\sigma(p_1, \dots, p_k))$ and  
%$t=\text{rhs}_M(q,\sigma,\<p_1,\dots, p_k>)$, any state call $\<q',x_i>$ 
%in $t$ is \emph{compatible} with a set 
%$Z \subseteq Y_m$ if, for all $s_i \in L_{p_i}$, the sequence nodes in 
%$t[\![\<q',x_i>\leftarrow \lcop{M_{q'}(s_i)}_{Y(q',p_i)}]\!]$ contain no 
%parameters from $Z$. 
%\end{definition}

The special first-order substitution is
the same as the normal one
except that it gives special treatment to \(Y\)-nodes
which is replaced by \(Y\)-nodes contains all parameters occurring 
in trees to be substituted for the parameters in the original \(Y\)-nodes.
%
The special second-order substitution is
the same as the normal one
except that the special first-order substitution is applied
for each involved first-order substitution.


\begin{lemma}\label{lm:rhs}
Let $M$ be a nondeleting mttr as before.
Let $q\in Q$, $\sigma\in\Sigma^{(k)}$, and
$p_1,\dots,p_k\in P$. Let $p=h(\sigma(p_1, \dots, p_k))$ and 
$t=\text{rhs}_M(q,\sigma,\<p_1,\dots, p_k>)$. 
Let $s_1 \in L_{p_1}, \dots, s_k \in L_{p_k}$. By $[\![.]\!]^{\$}$ we
denote the substitution $[\![\<q',x_i>\leftarrow \lcop{M_{q'}(s_i)}_{Y(q',p_i)} \mid q'\in Q, 
i \in [k]]\!]^{\$}$ and by $[\![M]\!]$ we denote 
$[\![\<q',x_i>\leftarrow M_{q'}(s_i) \mid q'\in Q, i \in [k]]\!]$.
\begin{enumerate}
\item[(1)] If $y\in Y(q,p)$ and $y$ occurs in $t$ in the $j$-th argument 
of a node $\<q',x_i>$ for $q' \in Q$ and $i\in [k]$, then $y_j \in Y(q',p_i)$. 
%If $y\in Y(q,p)$ and $y$ occurs in  $t_j$ ($j\in[m]$), then $y_j\in Y(q',p_i)$.
\item[(2)] No $Y$-node in $t[\![.]\!]\su$ intersects $Y(q,p)$. 
%Any state call $\<q',x_i>$ in $t$ is compatible with $Y(q,p)$. 
\item[(3)] $\lcop{t[\![.]\!]\su}_{Y(q,p)} = \lcop{t[\![M]\!]}_{Y(q,p)}$
%For all input trees $s_i\in L_{p_i}$, we have: ~~~~
%$\lcop{t[\![\dots]\!]}_{Y(q,p)} = \lcop{t[\![\lcop{\dots}]\!]}_{Y(q,p)}$ \\
%where $[\![\dots]\!]$ denotes $[\![\<q',x_i>\leftarrow M_{q'}(s_i)]\!]$ \\
%and $[\![\lcop{\dots}]\!]$ denotes $[\![\<q',x_i>\leftarrow \lcop{M_{q'}(s_i)}_{Y(q',p_i)} ]\!]$. 
\end{enumerate}
\end{lemma}
\begin{proof}
If some $y_j\notin Y(q',p_i)$ then $\lcop{M_{q'}(L_{p_i})}_{y_j}$ is 
infinite and, if $y$ occurs in $t_j$ ($j\in[m]$), then 
$\lcop{M_{q}(L_{p})}_{y}$ is also infinite and $y\notin Y(q,p)$. 
So~(1)~holds. 

%(2)~is a consequence of~(1).
%Alternative proof of (2):
If $y \in Y(q,p)$ occurs in a $Y$-node of $t[\![.]\!]\su$, 
then it occurs in $t$ in the $j$-th argument of a node $\<q',x_i>$ with 
$y_j \notin Y(q',p_i)$, which contradicts~(1). 
So~(2)~holds. 

%As a consequence of~(1), parameter nodes and inner nodes are identical in 
%$\lcop{t[\![\dots]\!]}_{Y(q,p)}$ and 
%$\lcop{t[\![\lcop{\dots}]\!]}_{Y(q,p)}$. 
%Sequence nodes are also identical as a consequence of Lemma~\ref{lm:nd}(2). 
%Therefore~(3)~holds. 
%Alternatice proof of (3)
%%% Original proof FROM HERE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Both $\lcop{t[\![M]\!]}_{Y(q,p)}$ and 
%$\lcop{t[\![.]\!]\su}_{Y(q,p)}$ contain three types of nodes: 
%parameter nodes of the form $y\in Y(q,p)$, inner nodes and $Y$-nodes. 
%As a consequence of~(1), paths to parameters nodes are identical in 
%$\lcop{t[\![M]\!]}_{Y(q,p)}$ and $\lcop{t[\![.]\!]\su}_{Y(q,p)}$, 
%and the same is true of the inner nodes along such paths. 
%$Y$-nodes are also identical as a consequence of Lemma~\ref{lm:nd}(2) and 
%of our definition of special second-order substitutions. 
%So~(3)~holds. 
%%% Original proof TO HERE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The statement~(3) is proved by induction on \(t\).
The cases of \(t=y_j\) and \(t=\gamma(t_1,\dots,t_n)\) are easy.
In the case of \(t=\<q',x_i>(t_1,\dots,t_m)\), we have
\begin{align*}
\lcop{t[\![.]\!]\su}_{Y(q,p)}
&=
\lcop{
\lcop{M_{q'}(s_i)}_{Y(q',p_i)}[y_j\leftarrow t_j[\![.]\!]\su\mid j\in[m]]\su
}_{Y(q,p)}
\\&=
\lcop{
\lcop{M_{q'}(s_i)}_{Y(q',p_i)}[y_j\leftarrow t_j[\![M]\!]\mid j\in[m]]\su
}_{Y(q,p)}
\\&=
\lcop{
M_{q'}(s_i)[y_j\leftarrow t_j[\![M]\!]\mid j\in[m]]
}_{Y(q,p)}
\\&=
\lcop{t[\![M]\!]}_{Y(q,p)}\text.
\end{align*}
%where the induction hypothesis and Lemma~\ref{lm:nd}(2) are used.
%
%Another alternatice proof of (3)
%To prove~(3)~we look at the $Y(q,p)$-skeleta of $t[\![\dots]\!]$ and 
%$t[\![\lcop{\dots}]\!]$. Those contain three types of nodes: 
%parameter nodes of the form $y\in Y(q,p)$, inner nodes (which are along 
%the paths to parameter nodes), and sequence nodes. Paths to parameters nodes 
%are identical in $t[\![\dots]\!]$ as in $t[\![\lcop{\dots}]\!]$ and so 
%are the inner nodes along such paths. Sequence nodes are also identical as a 
%consequence of Lemma~\ref{lm:nd}(2). 
\qed
\end{proof}

\input{constr_plus_examples.tex}

\subsection{Correctness Proof and Termination of Iteration}
\label{sect:corr}

Here we prove the correctness of transducer $\pi(M)$ that was defined
in Definition~\ref{df_depth_proper}. Lemma~\ref{lm:corr} establishes
the correctness of the look-ahead, relates the states of $\pi(M)$ to those
of $M$, and shows that the transducer $\pi(M)$ is nondeleting.
The latter is needed, so that the construction of $\pi$ can be carried
out iteratively (recall from Definition~\ref{df_depth_proper} that $M$ is
required to be nondeleting, in order to construct $\pi(M)$).


\begin{lemma}
\label{lm:corr}
Let $M$ be a nondeleting mttr and $N=\pi(M)$ be the mttr of
Definition~\ref{df:pi}, both with the tuples as in that definition. 
Let $s\in T_\Sigma$ with $\hat{h'}(s)=(p,\varphi)$.
Then
\begin{enumerate}
\item[(1)] $p=\hat{h}(s)$,
\item[(2)] $\forall q\in F_p$: $\varphi(q)=\lcop{M_q(s)}_{Y(q,p)}$, 
\item[(3)] $\forall q\in Q$: $N_q(s)=M_q(s)$,
\item[(4)] $\forall q\in F_p$ and $u\in V(t)$ with $t=\varphi(q)$ and
$t/u=\{y_{j_1},\dots,y_{j_n}\}$ with \\
$j_1<\cdots <j_n$:
$N_{[q,p,t,u]}(s)=M_q(s)/u[y_{j_\nu}\leftarrow y_\nu\mid\nu\in[n]]$, and
\item[(5)] the mttr $N$ is nondeleting.
\end{enumerate}
\end{lemma}
\begin{proof}
All the statements are proven by induction on the structure of $s$.
Let $s=\sigma(s_1,\dots,s_k)$ with $\sigma\in\Sigma^{(k)}$,
$k\geq 0$, and $s_1,\dots,s_k\in T_\Sigma$.
For $i\in[k]$ let $\hat{h'}(s_i)=(p_i,\varphi_i)$.
By the definition of $h'$, $p=h_\sigma(p_1,\dots,p_k)$, which 
is equal to $\hat{h}(s)$.
Thus, Statement~(1) holds.
For Statement~(2) let $q\in F_p$: 
Then $\varphi(q)$ is defined as 
$\lcop{\zeta[\![\varphi_i]\!]\su}_{Y(q,p)}$ where 
$\zeta=\text{rhs}_M(q,\sigma,\<p_1,\dots,p_k>)$
and
$[\![\varphi_i]\!]\su$ denotes the special substitution
$[\![ \< q',x_i>\leftarrow \varphi_i(q')\mid q'\in F_{p_i}, i\in[k]]\!]\su$.
By induction, $\lcop{\zeta[\![\varphi_i]\!]\su}_{Y(q,p)}$ equals
$\lcop{\zeta[\![ \< q',x_i>\leftarrow \lcop{M_{q'}(s_i)}_{Y(q',p_i)}
\mid q'\in F_{p_i}, i\in[k]]\!]\su}_{Y(q,p)}$.
By Lemma~\ref{lm:rhs}(3) the latter equals
$\lcop{\zeta[\![ \< q',x_i>\leftarrow M_{q'}(s_i)
\mid q'\in F_{p_i}, i\in[k]]\!]}_{Y(q,p)}
=\lcop{M(s)}_{Y(q,p)}$.


We now prove Statement~(3).
Let $q\in Q$.
Then $N_q(s)=\zeta[\![ . ]\!][\![N]\!]$, 
where 
$\zeta=\text{rhs}_M(q,\sigma,\<p_1,\dots,p_k>)$,
$[\![ . ]\!]$ is the substitution as in the construction, and
$[\![N]\!]=
[\![ \<r,x_i>\leftarrow N_r(s_i)\mid r\in Q',i\in[k] ]\!]$.
%
By the induction hypothesis of Statement~(2), we can replace
$\varphi_i(q')$ by $\lcop{M_{q'}(s_i)}_{Y(q',p_i)}$ in the
substitution $[\![ . ]\!]$. This gives
\begin{multline*}
\zeta
[\![ \<q',x_i>\leftarrow \lcop{M_{q'}(s_i)}_{Y(q',p_i)}
[
u'\leftarrow [q',p_i,\varphi_i(q'),u'](y_{j_1},\dots,y_{j_n})\mid \\
\varphi_i(q')/u'=\{y_{j_1},\dots,y_{j_n}\},
j_1<\cdots <j_n]
\mid q'\in F_{p_i},
i\in[k] ]\!]
[\![ N ]\!].
\end{multline*}
This can be written as 
$\zeta[\![.]\!][\![ H ]\!] [\![ Q ]\!]$,
where
$[\![ H ]\!]=[\![\< q',x_i>\leftarrow N_{q'}(s_i)\mid q'\in H,i\in[k] ]\!]$
and
$[\![ Q ]\!]  = 
[\![\< q',x_i>\leftarrow N_{q'}(s_i)\mid q'\in (Q \setminus F_{p_i}),i\in[k] ]\!]$.
%
By induction of Statement~(4) the substitution $[\![ H]\!]$ replaces the 
subtree $[q',p_i,\varphi_i(q'),u'](y_{j_1},\dots,y_{j_n})$ by the tree 
$M_{q'}(s_i)/u[y_{j_\nu}\leftarrow y_\nu\mid\nu\in[n]]
[y_\nu\leftarrow y_{j_\nu}\mid\nu\in[n]]=M_{q'}(s_i)/u$. 
Thus we obtain:
\begin{multline*}
\zeta
[\![ \<q',x_i>\leftarrow \lcop{M_{q'}(s_i)}_{Y(q',p_i)}
[
u'\leftarrow M_{q'}(s_i)/u'\mid 
u'\in\mathcal{U}(\lcop{M_{q'}(s_i)}_{Y(q',p_i)})]\\
\mid q'\in F_{p_i},
i\in[k] ]\!] 
[\![ Q ]\!]
\end{multline*}
By Lemma~\ref{lm:nd} (for $Z=Y(q',p_i)$ and $t=M_{q'}(s_i)$)
the tree on the right of the arrow
in the leftmost second-order substitution equals $M_{q'}(s_i)$.
We have:
\[
\zeta
[\![ \<q',x_i>\leftarrow M_{q'}(s_i)\mid q'\in F_{p_i},i\in[k] ]\!] 
[\![\< q',x_i>\leftarrow N_{q'}(s_i)\mid q'\in Q \setminus F_{p_i},i\in[k] ]\!].
\]
By induction of Statement~(3), $N_{q'}(s_i)=M_{q'}(s_i)$ for
$q\in Q \setminus F_{p_i}$. This gives us exactly $M_q(s)$, by the definition
of the semantics of mttrs. 
Thus,
\begin{equation}\label{eq:MN}
N_q(s)=\zeta[\![ . ]\!][\![N]\!]=M_q(s).
\end{equation}
This concludes the proof of Statement~(3).


We now prove Statement~(4).
Let $q\in F_p$ and $u\in V(t)$ with $t=\varphi(q)$ 
and $t/u\subseteq Y$.
By the definition of the rules for the helper states, 
$N_{[q,p,t,u]}(s)=(\zeta[\![ . ]\!])/u[\![ N ]\!][y]$
where $t/u=\{y_{j_1},\dots,y_{j_n}\}$, $j_1<\cdots <j_n$, and 
$[y]=[y_{j_\nu}\leftarrow y_\nu\mid\nu\in[n]]$.
It follows from Lemma~\ref{lm:rhs}(1) that if $\<q',x_i>$ occurs in 
$\zeta=\text{rhs}_M(q,\sigma,\langle p_1,$ $\dots,p_k\rangle)$
and $q\in F_p$, then $q'\not\in Q \setminus F_{p_i}$.
Hence, every proper ancestor
$v$ of $u$ is labeled by a symbol in $\Delta$, i.e.,
$(\zeta[\![.]\!][y])[v]\in\Delta$. 
This implies that we can move the ``$/u$'' operation of 
taking the subtree at node $u$
to the right (after the application of the substitution $[\![ N ]\!]$)
in the above displayed formula.
We obtain 
$\zeta[\![ . ]\!][\![ N ]\!]/u[y]$.
By the right equation in Formula~\ref{eq:MN}, this equals
$M_q(s)/u[y]$.

To prove Statement~(5), let $q\in Q^{(m)}$, $m\geq 0$.
Then 
\[
\zeta'=\text{rhs}_N(q,\sigma,\< (p_1,\varphi_1),\dots,(p_k,\varphi_k)>)=
\zeta[\![.]\!],
\]
where 
$\zeta=\text{rhs}_M(q,\sigma,\<p_1,\dots,p_k>)$ and
$[\![.]\!]$ is as before. 
By Statement~(2), $[\![.]\!]$ substitutes occurrences of 
$\<q',x_i>$ with $i\in[k]$ and $q'\in F_{p_i}$ by 
the tree $\lcop{M_{q'}(s_i)}_{Y(q',p_i)}$ in which leaves
labeled by $Z\subseteq Y_m$ are replaced by $\<q_H,x_i>(y_{j_1},\dots,
y_{j_n})$ with $Z=\{y_{j_1},\dots,y_{j_n}\}$.
By Lemma~\ref{lm:nd}(2) this implies that 
$y_j$ occurs in $\zeta'$ for each $j\in[m]$.
\qed
\end{proof}

\input{termination}


==> introduction.tex <==
\section{Introduction}

Tree transducers are fundamental devices in theoretical computer science.
%automata theory.
They generalize the finite state transductions from strings to (finite, ranked) trees and
were invented in the 1970s in the context of compiler theory and mathematical linguistics.
The most basic such transducers are the top-down tree
transducer~\cite{DBLP:journals/jcss/Thatcher70,DBLP:journals/mst/Rounds70}
and the bottom-up tree transducer~\cite{th70}, see also~\cite{DBLP:journals/mst/Engelfriet75}.
These transducers traverse their input tree once, but may process subtrees in several copies.
It is well known that these transducers have \emph{linear height increase} (``LHI''),
see e.g.~\cite{DBLP:series/eatcs/FulopV98}.

In this paper we deal with a more powerful kind of tree transducer:
the macro tree transducer~\cite{DBLP:journals/jcss/EngelfrietV85} (``mtt'').
Mtts can be seen as particularly simple functional
programs on trees restricted to primitive recursion via (input) tree pattern matching.
Alternatively, mtts can be seen as context-free tree grammars
(introduced in~\cite{DBLP:journals/mst/Rounds70} as ``context-free dendrogrammars'';
see also~\cite{fis68,DBLP:journals/jcss/EngelfrietS77,DBLP:journals/jcss/EngelfrietS78}
and~\cite[Section~15]{DBLP:reference/hfl/GecsegS97}),
the nonterminals of
which are controlled by a top-down tree storage (in the spirit of~\cite{DBLP:journals/corr/Engelfriet14}).

It is an open problem, if it is decidable for a given mtt whether or not
its translation can be realized by a top-down tree transducer
(with ``origin'' semantics, this problem was shown to be decidable~\cite{DBLP:journals/iandc/FiliotMRT18}).
As mentioned above, it is a necessary condition for the mtt to have
linear height increase (``LHI''). 
This raises the question, can we decide for a given
mtt, whether or not its translation has LHI?
Here we give an affirmative answer to this question.
%
---
It is also an open problem, if it is decidable for a given mtt whether or not
its translation can be realized by an attributed tree 
transducer~\cite{DBLP:journals/mst/Knuth68,DBLP:journals/actaC/Fulop81} (``att'').
It is well-known that atts have \emph{linear size-to-height increase} (``LSHI''), 
see, e.g.,~\cite{DBLP:series/eatcs/FulopV98}. 
This raises the question, can we decide for a given
mtt, whether or not its translation is of LSHI?
Also to this question we give an affirmative answer.
Note that it was conjectured in~\cite{DBLP:journals/siamcomp/EngelfrietM03}
that the methods of that paper
could be adapted to give such an affirmative answer.

Let us now discuss our results in more detail.
To decide both the LHI and LSHI properties, we introduce a new normal form
called ``depth proper''. An mtt is depth proper if each parameter of every 
(reachable) state
appears at infinitely many different depths (for different input trees).
The idea of our construction is to eliminate 
parameters that only appear at bounded depths; we use regular
look-ahead to determine which bounded paths to output at a given moment.
Since in this way we may generate output ``earlier'' than the original transducer,
new ``helper states'' need to be introduced which continue the translation at
the correct input nodes. Both issues, the change of look-ahead and the introduction
of new states may cause the newly constructed transducer \emph{not} to be depth proper.
For this reason our construction has to be iterated before a depth proper mtt
is obtained.

To understand the idea of the construction, let us consider a simple example.
We consider input and output trees over a binary symbol $f$ and the
nullary symbol $a$ and an mtt with the following rules.
\[
\begin{array}{lcl}
q_0(f(x_1,x_2)) &\to& f(q_1(x_2), q_2(x_2, q_{\text{id}}(x_1)))\\
q_0(a)&\to& a\\  
q_1(f(x_1,x_2)) &\to& q_{\text{id}}(x_1)\\
q_1(a)&\to& a\\  
q_2(f(x_1,x_2),y_1) &\to& f(y_1, q_0(x_2))\\
q_2(a,y_1) &\to& f(y_1, a)\\
q_{\text{id}}(f(x_1,x_2)) &\to& f(q_{\text{id}}(x_1), q_{\text{id}}(x_2))\\
q_{\text{id}}(a) &\to& a
\end{array}
\]
The transducer realizes the following translation:
\[
f(t_1, f(t_2, \underbrace{f(t_3, f(t_4, \dots ))}_{t} )) \Rightarrow
f(t_2, f(t_1, f(t_4, f(t_3, \dots ))))
\]
Let us consider in detail how the rules of the mtt are applied 
to produce as output first the tree $t_2$ and then the tree $t_1$:
\[
\begin{array}{cl}
& q_0(f(t_1,f(t_2,t)))\\
\Rightarrow_{\text{first rule}} & f( q_1(f(t_2,t)), q_2(f(t_2,t), q_{\text{id}}(t_1)))\\
\Rightarrow_{\text{second rule}} & f( q_{\text{id}}(t_2), q_2(f(t_2,t), q_{\text{id}}(t_1)))\\
\Rightarrow_{\text{last two rules}}^* & f( t_2, q_2(f(t_2,t), q_{\text{id}}(t_1)))\\
\Rightarrow_{\text{third rule}} & f( t_2, f(q_{\text{id}}(t_1),q_0(t))\\
\Rightarrow_{\text{last two rules}}^* & f( t_2, f(t_1,q_0(t)))
\end{array}
\]  
%Let us consider the first (top-most) rule: the state $q_1$ produces
%the tree $t_2$. The state $q_2$ takes in its parameter argument the
%tree $t_1$ (produced by the call $q_{\text{id}}(x_1)$).
%At the \emph{next} node of the right-comb of the input tree
%the state $q_2$ outputs $f(t_1, t)$ where $t$ is the translation of the transducer 
%for the tree $f(t_3, \dots)$.
Parameters of an mtt are always instantiated by output trees.
In the example, the parameter $y_1$ of state $q_2$ is instantiated by the output
tree that is produced by the call $q_{\text{id}}(t_1)$.
Observe further, that state $q_2$ is 
\emph{not} depth proper: each tree that it outputs is of the form
$f(y_1, t)$ where $t$ does not contain the parameter $y_1$.
The idea of our construction is to replace each occurrence of state $q_2$ in
the right-hand side of any rule by this tree ``fragment'', where at the 
position of $t$ there will be the new ``helper state'' $[q_2,2]$. 
The path ``2'' indicates that this state should produce the tree at the second
child position of the output tree produced by $q_2$.
We obtain the following (the rules of $q_0,q_1$ and input $a$ are as before):
\[
\begin{array}{lcl}
q_0(f(x_1,x_2)) &\to& f(q_1(x_2), f(q_{\text{id}}(x_1), [q_2,2](x_2) )) \\
q_1(f(x_1,x_2)) &\to& q_{\text{id}}(x_1)\\
{[q_2,2]}(f(x_1,x_2)) &\to& q_0(x_2)\\
{[q_2,2]}(a) &\to& a\\
q_{\text{id}}(f(x_1,x_2)) &\to& f(q_{\text{id}}(x_1), q_{\text{id}}(x_2))\\
q_{\text{id}}(a) &\to& a
\end{array}
\]
It should be clear that the new transducer is equivalent to the original one.
Moreover, the new transducer uses no parameters whatsoever, therefore it is
depth proper.

Given a depth proper mtt, we can decide the LSHI property as follows.
We consider input trees which contain exactly one special marked input leaf
(it will be marked by a state $p$ of the look-ahead automaton, to act as a place-holder for
any input tree for which the look-ahead automaton arrives in state $p$).
For such input trees, the mtt produces output trees which only contain nested state calls
to the special input leaf. The original transducer has LSHI if and only if the
range of this transducer is finite (which is known to be decidable~\cite{DBLP:journals/iandc/DrewesE98}).
In a similar way we can decide LHI: here we consider input trees with multiple
marked input leaves.
To show that if such ranges are not finite, then the translation does not
have LSHI (or LHI), is done via pumping arguments (which use depth properness);
these pumping arguments are similar to the ones used in~\cite{DBLP:journals/siamcomp/EngelfrietM03}
to show that it is decidable whether or not an mtt has \emph{linear size increase} (LSI).

%In fact, it is known that
If we restrict the translations of mtts to LSI,
then we obtain exactly the MSO definable tree translations~\cite{DBLP:journals/siamcomp/EngelfrietM03}.
Moreover, LSI is decidable for mtts
(it can even be decided for compositions of mtts, and if so,
then the translation is effectively MSO definable~\cite{DBLP:journals/acta/EngelfrietIM21}).
To decide LSI,
the given mtt is first transformed into ``proper'' normal form.
Properness guarantees that 
(1)~each state (except possibly the initial state) produces
infinitely many output trees (this is called ``input proper''),
and that 
(2)~each parameter of a state is instantiated with infinitely many
distinct argument trees (this is called ``parameter proper'').
Note that input properness is a 
generalization of the proper form of~\cite{DBLP:journals/iandc/AhoU71}.
Once in proper normal form, it suffices to check if the transducer
is ``finite copying''. This means that 
(a)~each node of each input tree is processed only a bounded number of times
and that
(b)~each parameter of every state is copied only a bounded number of times. 
Both of these properties can be reduced to the finiteness problem
of ranges of compositions of mtts~\cite{DBLP:journals/iandc/DrewesE98}.
It is also proved (via complicated pumping arguments)
that if a proper mtt is \emph{not} finite copying, then its
translation is \emph{not} of LSI.

Note that the original proof of the proper form of~\cite{DBLP:journals/iandc/AhoU71}
was not correct, because they had not realized that their construction needed to be iterated.
In~\cite{DBLP:journals/siamcomp/EngelfrietM03} it was shown that at most
$|Q|$-many iterations (where $Q$ is the set of states of the original given mtt)
yield an input-proper mtt.
As mentioned before, termination in our depth proper normal form is more complex,
because new states are also introduced.
%We prove termination by a 
%K{\"o}nig's Lemma like argument.
%
%
%
%
\iffalse
We say that the mtt has the ``finite nesting'' property, if
there is a bound on the number of nested state calls that appear on any path of such output trees.

We can decide whether or not an mtt is finite nesting, similar as before: we change the mtt
to nondeterministically output any path of nested states of any such output tree. The 
original mtt is finite nesting if and only if the range
of this transducer is finite (the latter is decidable, as mentioned above).
We can also show that is the mtt is \emph{not} finite nesting, then the given translation
if \emph{not} LSHI.

Technically speaking all our mtts are always equipped with look-ahead. 
Two issues that arise in our construction in general are:
(\emph{i.}) the

In the case of input-properness, only the look-ahead changes in each iteration of the construction.
Our construction of a depth proper mtt also needs to be iterated due to the change of
look-ahead, however, we also add new states in each iteration. This complicates the 
termination proof and we are not able to present a simple bound such as $|Q|$ for our iteration. 

The proof of this normal form is similar to the one of input-properness, but
more complicated.
\fi


==> termination.tex <==
%!TEX root = main.tex

% macros (will be moved later)

%\section{Termination of the procedure}

We now show that the iteration of the construction $\pi(M)$ will
terminate with a transducer that is depth proper.
%For an arbitrary transducer $M$ and a look-ahead state $p$ of $M$ we define
%the set $U_p$ of states $q$ such that $(q,p)$ us unreachable as follows''
%\[
%U_p = \{ q\in Q\mid (q,p)\text{ is unreachable in }M\}.
%\]
%Note that $M$ is depth proper if $F_p\subseteq U_p$ for every look-ahead state $p$ of $M$.
%
First, let us discuss what property a single iteration of $\pi$ ensures.
Let $p\in P$.
Note that the set $F_p$ is defined independently of reachability, i.e.,
$F_p$ may contain states $q$ such that $(q,p)$ is \emph{not} reachable.
Let $\varphi$ such that $(p,\varphi)\in P'$.
Then
\[
F_p\subseteq F_{(p,\varphi)}.
\]
This inclusion follows from Lemma~\ref{lm:corr} as follows:
let $s\in L_{(p,\varphi)}$ and let $q\in F_p$ be of rank $m$.
The latter means that there exists a $j\in[m]$ and a number $n$ 
such that every occurrence of $y_j$ in $M_q(s')$ is
at depth $\leq n$ for every $s'\in L_p$.
By Lemma~\ref{lm:corr}~(1), $s\in L_p$ and by Lemma~\ref{lm:corr}~(3),
$N_q(s)=M_q(s)$. Thus, every occurrence of $y_j$ in $N_q(s)$ also
occurs at depth $\leq n$. Hence, $q\in F_{(p,\varphi)}$.

We now consider reachability.
We say that a state $q$ is \emph{depth proper}, if for all $p\in P$ such that
$(q,p)$ is reachable, $q\not\in F_p$.
If $q\in F_p$, then for all $\varphi$ such that $(p,\varphi)\in P'$ it holds that
$(q,(p,\varphi))$ is not reachable.
This property follows immediately from the definition of look-ahead and the rules of $\pi(M)$:
the substitution $[\![.]\!]$ replaces each state call $\<q',x_i>$ with $q\in F_{p_i}$ by
a tree that does not contain states of $Q$.
So, if $(q,(p,\varphi))$ is reachable, then $q\not\in F_p$;
however, it may be that $q\in F_{(p,\varphi)}$, which means that $q$ is
not depth proper. It means that if $F_{(p,\varphi)}=F_p$ for
all $(p,\varphi)\in P'$, then all states $q\in Q$ are depth proper.
Let $Q_0=Q$ and consider now the iterated application of $\pi$.
Clearly, after some iterations of $\pi$, it will hold that
$F_{(p,\varphi)}=F_p$ for all $(p,\varphi)\in P'$.
To see this, consider the chain of inclusions
\[
F_p\cap Q_0 \subseteq F_{(p,\varphi_1)}\cap Q_0 \subseteq \dots \subseteq
   F_{(p,\varphi_1,\dots,\varphi_k)}\cap Q_0 \subseteq \dots
\]
for any maps \(\varphi_i\) introduced in the look-ahead of \(\pi^i(M)\).
Since \(Q_0\) is finite, the chain contains only finitely many strict inclusions.
Hence there is a minimal \(n\) such that 
\( F_{(p,\varphi_1,\dots,\varphi_n)}\cap Q_0 = F_{(p,\varphi_1,\dots,\varphi_{n'})} \cap Q_0 \)
for any \(n'>n\).

Consider a tree with an artificial root node which contains all such chains, i.e.,
for each $p\in P$ there is exactly one child of the root node labeled $F_p$, and 
a node labeled $F_p$ has children labeled $F_{(p,\varphi)}$ for each $(p,\varphi)\in P'$, etc. 
Moreover, a node labeled $F_{(p,\varphi_1,\dots,\varphi_n)}$ as in the chain above
is a leaf of this tree.
Since each node of this tree is finitely branching (because $P'$ is finite) and each
path has finite length, we know by K{\"o}nig's lemma that tree is finite.
Thus, if $d$ is the depth of this tree, for the 
mttr $M'=\pi^d(M)$, all states in $Q_0$ are depth proper.

Let $m$ be the maximal rank of the states in $Q_0$.
Since all helper states are of rank $<m$, we know that
$M'$ contains no improper states of rank $\geq m$.
We now proceed in the same fashion and construct a transducer $M''=\pi^{n'}(M')$
which contains no improper states of rank $\geq (m-1)$.
In a similar way we 
eventually obtain an mttr for which \emph{all states} are depth proper
(and which is equivalent to $M$).
Thus, even though we do not constructively derive a precise bound, we know that
after \emph{some} number of applications of $\pi$ we are sure to obtain
a depth proper mttr.

%\begin{lemma}\label{lm:term}
%Let \(M\) be a nondeleting mttr with improper states of rank at most \(m\).
%There exists \(N\) such that, for all $n \geq N$, 
%any reachable improper state call of \(\pi^n(M)\) has rank at most \((m-1)\).
%old version: (I only added the ", for all $n \geq N$, " and " call ")
%Let \(M\) be a nondeleting mttr with improper states of rank at most \(m\).
%There exists \(n\) such that 
%any improper state of \(\pi^n(M)\) has rank at most \((m-1)\).
%\end{lemma}
%
%\begin{proof}
%From the construction, 
%every look-ahead of \(\pi^k(M)\) has the form: \((p,\varphi_1,\dots,\varphi_k)\)
%with a look-ahead state \(p\) of \(M\).
%Let \(Q_0\) be the set of states of \(M\). 
%BLAH
%Note that the construction $\pi$ may introduce new states, called 
%\emph{helper states}, but those states have rank at most $(m-1)$. 
%So we only need to prove that no state in $Q_0$ is called improperly after enough 
%iterations of $\pi$, i.e.\ there exists $N \in \N$ such that for all $n \geq N$ and 
%look-ahead state $(p,\varphi_1, \dots, \varphi_n)$ of $\pi^n(M)$: $Q_0 \cap F_{(p, \varphi_1, \dots, \varphi_{n})} = Q_0 \cap U_{(p, \varphi_1, \dots, \varphi_{n})}$. 
%
%For each $p$, we consider the unranked tree whose nodes of depth $n$ are the 
%look-ahead states of $\pi^n(M)$ of the form $(p,\varphi_1, \dots, \varphi_n)$, 
%rooted in look-ahead state $p$, and such that the parent node of a node 
%$(p,\varphi_1, \dots, \varphi_n)$ is $(p,\varphi_1, \dots, \varphi_{n-1})$. 
%This tree has no node of infinite rank. 
%From this tree we remove all branches without look-ahead states for which there 
%exists a reachable improper state in $Q_0$ (i.e.\ such that 
%$Q_0 \cap F_{(p,\varphi_1, \dots, \varphi_n)} \setminus U_{(p,\varphi_1, \dots, \varphi_n)} \neq \emptyset$). 
%$\pi$ can introduce helper states of rank at most $(m-1)$, so we can conclude 
%by using K{\"o}nig's Lemma on this tree. We now only need to prove that the tree 
%contains no infinite branch. 
%
%BLAH
%
%
%\qed
%\end{proof}

\begin{theorem}
  \label{th:proper}
For every mttr \(M\), there is a proper mttr \(M'\) equivalent to \(M\).
\end{theorem}
%
\begin{proof}
There is a nondeleting mttr \(M_0\) equivalent to \(M\) 
(\cite{DBLP:journals/iandc/EngelfrietM99} or Proposition~\ref{prop:nondeleting}).
We repeatedly construct equivalent transducers $\pi(M)$, $\pi(\pi(M))$, etc.
until a proper mttr is obtained (which is decidable by
Lemma~\ref{lm:dec}). The repetition terminates 
(first eliminating all reachable calls of improper states of the highest rank $m$, then
those or rank $m-1$, etc.).
\qed
\end{proof}

